Underwater Image Restoration via Contrastive Learning and a Real-world Dataset

Underwater image restoration is of significant importance in unveiling the underwater world. Numerous techniques and algorithms have been developed in the past decades. However, due to fundamental difficulties associated with imaging/sensing, lighting, and refractive geometric distortions, in capturing clear underwater images, no comprehensive evaluations have been conducted of underwater image restoration. To address this gap, we have constructed a large-scale real underwater image dataset, dubbed `HICRD' (Heron Island Coral Reef Dataset), for the purpose of benchmarking existing methods and supporting the development of new deep-learning based methods. We employ accurate water parameter (diffuse attenuation coefficient) in generating reference images. There are 2000 reference restored images and 6003 original underwater images in the unpaired training set. Further, we present a novel method for underwater image restoration based on unsupervised image-to-image translation framework. Our proposed method leveraged contrastive learning and generative adversarial networks to maximize the mutual information between raw and restored images. Extensive experiments with comparisons to recent approaches further demonstrate the superiority of our proposed method. Our code and dataset are publicly available at GitHub.

==> tables/equation.tex <==
 \begin{table*}[!htbp]
  \centering
%   \fontsize{11}{4}\selectfont
    \begin{tabular}{lcl}
    \toprule
    \cr
    \textbf{Loss type}&\textbf{Equation No.}&\multicolumn{1}{c}{\textbf{Equation}}\cr
    \midrule
    Adversarial &6& 
    $\mathcal{L}_{\mathrm{GAN}}\left(G, D, X, Y\right) =\mathbb{E}_{y\sim{Y}}\left[(D(y))^2\right] +\mathbb{E}_{x\sim{X}}\left[\left(1-D(G(x))\right)^2]\right.$
    \cr
    Cross-entropy &7& 
    $ \ell\left(\boldsymbol{v}, \boldsymbol{v}^{+}, \boldsymbol{v}^{-}\right)= -\log( \frac{\exp \left(\boldsymbol cos({v},\boldsymbol{v}^{+}) / \tau\right)}{\exp \left(\boldsymbol cos({v},\boldsymbol{v}^{+}) / \tau\right)+\sum_{n=1}^{N} \exp \left(\boldsymbol cos({v},\boldsymbol{v}_{n}^{-}) / \tau\right)})$
    \cr   
    PatchNCE &8& 
    $\mathcal{L}_{\mathrm{PatchNCE}}(G,H,X)=
    \mathbb{E}_{\boldsymbol{x} \sim X} \sum_{l=1}^{L} \sum_{s=1}^{S_{l}} \ell\left(\hat{z}_{l}^{s}, \boldsymbol{z}_{l}^{s}, \boldsymbol{z}_{l}^{S \backslash s}\right)$
    \cr
    Identity &9& 
    $\mathcal{L}_{\text {Identity}}(G)=\mathbb{E}_{y \sim {Y} }\left[\|G(y)-y\|_{1}\right]$
    \cr   
    \bottomrule
    \end{tabular}
      \caption{Components of the full objective. We use least-square adversarial loss for equation 6. For equation 7, we use a noisy contrastive estimation framework to maximize the mutual information between inputs and outputs. The idea behind equation 7 is to correlate two signals, \ie, the \enquote{query} and its  \enquote{positive} example, in contrast to other examples in the dataset (referred to as  \enquote{negatives}). We map query, positive, and $N$ negatives to $K$-dimensional vectors and denote them $v, v^{+} \in R^{K}$ and $ v^{-} \in R^{N \times K}$, respectively. Note that $v_{n}^{-} \in R^{K}$ denotes the n-th negative. We set up an $(N+1)$-way classification problem and compute the probability that a  \enquote{positive} is selected over \enquote{negatives}. This can be expressed as a cross-entropy loss where $\operatorname{cos}(\boldsymbol{u}, \boldsymbol{v})=\boldsymbol{u}^{\top} \boldsymbol{v} /\|\boldsymbol{u}\|\|\boldsymbol{v}\|$ denotes the cosine similarity between $\boldsymbol{u}$ and $\boldsymbol{v}$. $\tau$ denotes a temperature parameter to scale the distance between the query and other examples, we use 0.07 as default. For equation 8, We select $L$ layers from $G_{enc}(X)$ and send them to a projection head $H_{X}$, embedding one image to a stack of feature $\left\{\boldsymbol{z}_{l}\right\}_{L}=\left\{H^{l}\left(G_{\mathrm{enc}}^{l}(\boldsymbol{x})\right)\right\}_{L}$, where $G_{\mathrm{enc}}^{l}$ represents the output of $l$-th selected layers. After having a stack of features, each feature actually represents one patch from the image. We denote the spatial locations in each selected layer as $s \in \{1,...,S_{l}\}$, where $S_{l}$ is the number of spatial locations in each layer. We select a query each time, refer the corresponding feature ("positive") as $\boldsymbol{z}_{l}^{s} \in \mathbb{R}^{C_{l}}$ and all other features (\enquote{negatives}) as $\boldsymbol{z}_{l}^{S \backslash s} \in \mathbb{R}^{\left(S_{l}-1\right) \times C_{l}}$, where $C_{l}$ is the number of channels in each layer. Two losses are introduced to prevent generator from unnecessary changes. Equation 9 is a $\ell_1$ Identity loss preserving the fidelity.}
  \label{tab:equations}
\end{table*}

